GPU Acceleration and Portability of the TRIMEG Code for Gyrokinetic Plasma Simulations using OpenMP

The field of plasma physics heavily relies on simulations to model various phenomena, such as instabilities, turbulence, and nonlinear behaviors that would otherwise be difficult to study from a purely theoretical approach. Simulations are fundamental in accurately setting up experiments, which can be extremely costly and complex. As high-fidelity tools, gyrokinetic simulations play a crucial role in discovering new physics, interpreting experimental results, and improving the design of next-generation devices. However, their high computational costs necessitate the use of acceleration platforms to reduce execution time. This work revolves around the TRIangular MEsh based Gyrokinetic (TRIMEG) code, which performs high-accuracy particle-in-cell plasma simulations in tokamak geometries, leveraging a novel finite element approach. The rise of graphical processing units (GPUs) constitutes an occasion to satisfy such computational needs, by offloading the most expensive portion of the code to the accelerators. The chosen approach features GPU offloading with the OpenMP API, which grants portability of the code to different architectures, namely AMD and NVIDIA. The particle pushing as well as the grid-to-particle operations have been ported to GPU platforms. Compiler limitations had to be overcome, and portions of the code were restructured to be suitable for GPU acceleration. Kernel performance was evaluated by carrying out GPU grid size exploration, as well as scalability studies. In addition, the efficiency of hybrid MPI-OpenMP offloading parallelization was assessed. The speedup of the GPU implementation was calculated by comparing it with the pure CPU version using different rationales. The Ion Temperature Gradient (ITG) mode was simulated using the GPU-accelerated version, and its correctness was verified in terms of the energy growth rate and the two-dimensional mode structures.

==> Chapter4/chapter4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%2345678901234567890123456789012345678901234567890123456789012345678901234567890
%        1         2         3         4         5         6         7         8
% THESIS CHAPTER

\chapter{GPU offloading of a 1D PIC Code}
\label{chap:fourth}
\ifpdf
    \graphicspath{{Chapter3/Figures/PNG/}{Chapter3/Figures/PDF/}{Chapter3/Figures/}}
\else
    \graphicspath{{Chapter3/Figures/EPS/}{Chapter3/Figures/}}
\fi

\section{Model Description}
A PIC code was developed to test GPU offloading on a smaller scale. The model considers a one-dimensional uniform plasma in a uniform magnetic field in the electrostatic limit, i.e., $\beta=0$. 
In the model, the ion response is described with the polarization density, and the only particle species considered is the kinetic electron. 
A high-level-of-abstraction perspective of the problem resolution is the following:

\begin{enumerate}
    \item compute the plasma density values in the \texttt{p2g} phase
    \item solve the field equation to get the perturbed field
    \item interpolate the field quantities on the grid to the particle positions in the \texttt{g2p} phase
    \item solve the equations of motion to evolve the particle positions and velocities in the particle pushing procedure
\end{enumerate}

The model solves the gyrokinetic quasi-neutrality equation, whose normalized form in three dimensions is the following \cite{lu2021development}:

\begin{equation} \label{Poisson Ampere equation}
    -\nabla_\perp\cdot g\nabla_\perp\delta\phi = C_p \delta N,
\end{equation}

\begin{equation}
    g = \sum_s M_s\frac{n_{0s}B_0^2}{\langle n \rangle B^2}\;,\;\delta N = \sum_se_s\frac{\delta n_s}{\langle n\rangle} \;\;,
\end{equation}
where $s$ denotes the particle species, $M_s=m_s/m_N$, $C_p = 1/\rho_N^2$, $B_0$ is the reference magnetic field, $\beta = 2\mu_0\langle n \rangle T_N/B_0^2$ and $\langle n\rangle$ is the average density. In the 1D case with uniform density, $\langle n \rangle=n$.
Let us decompose the perturbed field and density with a Fourier expansion, using complex exponentials as basis functions in one dimension.

\begin{align} \label{Fourier decomposition of perturbed field}
\delta\phi&=\sum_k\delta\phi_k e^{-ikx}, \\
\delta n &=\sum_k\delta N_k e^{-ikx}
\end{align}
where $k$ is the mode number, with a total of $N_k$ modes used by the model, valid for $\forall s$ particle species.

The equation for the magnetic vector potential is not considered, as the current simplified PIC model considers only the contribution given by the scalar electric potential, as previously mentioned. The normalized version of Eq.~\eqref{Poisson Ampere equation} that is actually solved in the model is given below:
\begin{equation}\label{actual poisson equation}
    \rho_N^2\nabla_\perp^2\delta\phi = -e \delta n_e
\end{equation}

We employ the Fourier decomposition described in Eq.~\eqref{Fourier decomposition of perturbed field} and obtain the following results:

\begin{equation}
    \rho_N^2 \nabla_\perp^2\delta\phi_ke^{ikx} = -e\delta n_ke^{ikx}\;\;\forall k = -N_k,\dots,N_k
\end{equation}

Now we shall decompose the single $n_k$ contribution by means of the particle-in-Fourier in the parallel direction:
\begin{equation}
    \delta n_{k} = \frac{1}{N_p}\sum_{p=1}^{N_p}e^{-ikx_p}
\end{equation}

Using this decomposition, from Eq.~\eqref{actual poisson equation} we obtain the following:
\begin{equation}
\rho_N^2\nabla_\perp^2 \delta\phi_ke^{ikx} = -ee^{ikx}\frac{1}{N_p}\sum_{p=1}^{N_p}e^{-ikx_p}
\end{equation}
The calculation of the second-order derivative yields the following:

\begin{equation}
    -\rho_N^2 k_\perp^2\delta\phi_k e^{ikx} = -\frac{e}{N_p}e^{ikx}\sum_{p=1}^{N_p}e^{-ikx_p}
\end{equation}
Therefore:
\begin{equation}
    \delta\phi_k = \frac{e}{\rho_N^2k_\perp^2}\sum_{p=1}^{N_p}e^{-ikx_p}
\end{equation}
where the complex exponential inside the summation can be decomposed using Euler's formula:
\begin{equation}
    \delta\phi_k = \frac{e}{\rho_N^2k_\perp^2}\sum_{p=1}^{N_p} \left[ \text{cos}(kx_p) - i\text{{sin}}(kx_p) \right]
\end{equation}

The normalized gyro center's equations of motion to compute the particle positions and velocities are the following:
\begin{eqnarray}
    \frac{dx}{dt}&=&v_\| \\
\label{EOM velocity}
    \frac{dv_{||}}{dt} &=&- \frac{\bar e_s}{M_e}\partial_{||}\delta\phi,
\end{eqnarray}
where the normalized particle species is $\bar e_s=e_s/e$, the normalized particle mass $M_e = m_s/m_N$, $\partial_{||} =\partial_x $ in the 1D case; note that the term depending on the magnetic vector potential has been neglected due to $\beta=0$.
As previously done, the perturbed potential can be decomposed using a Fourier expansion. However, it is necessary to impose that the imaginary part is equal to zero for variables in configuration space, which amounts to imposing the condition
$$
    \delta\phi(x)^*=\delta\phi(x)
$$
Take the complex conjugate of the expression in Eq.~\eqref{Fourier decomposition of perturbed field}
$$
\delta\phi(x)^*=\sum_k\delta\phi_k^*e^{-ikx}
$$
Label the index $k$ as $-k$
$$
\delta\phi(x)^*=\sum_{-k}\delta\phi_{-k}^*e^{ikx}
$$
By comparing the expression above with  Eq. \eqref{Fourier decomposition of perturbed field}, we obtain the reality condition 
$$
\delta\phi_k=\delta\phi_{-k}^*\;,
$$
which implies that the imaginary parts cancel out and the real parts add constructively, thus leading to
$$
\delta\phi(x)=2\sum_{k>0}\textbf{Re}\Big(\delta\phi_ke^{ikx}\Big)+\delta\phi_0
$$
Now we shall compute the spatial derivative of the latest expression for the perturbed field, which corresponds to
\begin{equation}\label{EOM spatial derivattive}
\partial_x\delta\phi=2\textbf{Re}\Big(\partial_x\Big(\delta\phi_ke^{ikx}\Big)\Big) = 2\textbf{Re}\Big(ik\delta\phi_ke^{ikx}\Big)
\end{equation}
We can treat the term $\delta\phi e^{ikx}$ separately:
\begin{align}
\delta\phi e^{ikx}&=(\delta\phi_R+\delta\phi_I)(\text{cos}(kx)+i\text{sin}(kx))\\
&=(\delta\phi_R \text{cos}(kx)-\delta\phi_I \text{sin}(kx))+i(\delta\phi_R \text{sin}(kx)+\delta\phi_I \text{cos}(kx))
\end{align}
Since only the real part is needed for the calculation of the spatial derivative in Eq. \eqref{EOM spatial derivattive}, we obtain the following:
\begin{equation}
    \partial_x\delta\phi = -2k((\delta\phi_R \text{sin}(kx)+\delta\phi_I \text{cos}(kx))
\end{equation}

Therefore, the gyro center's equation of motion for velocity in Eq.~\eqref{EOM velocity} becomes
\begin{equation}
    \frac{dv}{dt} = -\frac{e}{m}2k((\delta\phi_R \text{sin}(kx)+\delta\phi_I \text{cos}(kx))
\end{equation}

\section{Numerical Scheme and Code Implementation}
The numerical scheme that is used to push particles is the simplest, that is, forward Euler. It is an explicit first-order numerical scheme for solving ODEs and the most basic Runge-Kutta method. Specifically, the method is given by the following steps. First, compute the increment at the current time step:
$$\Delta \textbf{X}_1 = \Delta td_t\textbf{X}(\textbf{X}_t,\delta \phi_t),$$
where $d_t\textbf{X}=d\textbf{X}/dt$, $\textbf{X} = (\textbf{R},v_{||})$
Then, the value at the current time step is given by:
$$\textbf{X}(t+\Delta t)=\textbf{X}(t)+\Delta\textbf{X}_1$$
As forward Euler is an explicit method, it is conditionally stable with respect to the chosen time step. \\

The 1D PIC model has been developed in Fortran following previous work \cite{lu2021development}, with the upgrade leveraging GPU offloading with OpenMP.  The  constraints from the compiler for the GPU-offloading has also been considered when developing the GPU version of the code.  
The GPU version of the code is not part of this work, which features the compilation specifically for MI300A architecture, the evaluation of the model for different configuration parameters and the performance gain of the accelerated version with respect to the sequential one. The code has been developed to demonstrate the potential effectiveness of the GPU offloading approach for TRIMEG. To mimic the paradigm that is applied to the latter, the initialization phase is not accelerated on the GPU device. It mainly consists of sampling the Maxwellian distribution to get the initial particle positions and velocities. In TRIMEG it is already parallelized with MPI in an efficient way, besides it amounts to a very small percentage of the total execution time. The focus of the offloading is the gather-scatter scheme, which is described in the following pseudo-algorithm:  
\begin{verbatim}
init_particles_Maxwellian
do i:num_time_steps
    particle_deposition_to_grid
    solve_field_equation
    interpolate_grid_values_to_particles
    particle_push
enddo
\end{verbatim}

\section{Error convergence}
In gyrokinetic theory, energy is stored both in the electromagnetic field and in the particles. The Hamiltonian of an individual particle is not invariant, as the electromagnetic field fluctuates over time. For this reason, the total energy of the system is regarded as the conserved quantity. It is obtained as the sum of the kinetic energy of the particles and the energy stored in the electromagnetic field. The current 1D model includes only the electric field, hence why energy is stored only inside the electrostatic potential. The actual energy conservation depends on the numerical property of the integration method that is used to compute the evolution over time. In this case, the integration method is forward Euler, which is characterized by conditional stability. Therefore, the chosen time step is crucial to the precision with which the model conserves the total energy. In Fig. \ref{fig:energy-oscillation-over-time}, a plot of the energy oscillation over time for $10^7$ particle markers, a time step equal to 0.00003125 and a number of time steps equal to 4000.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/energy_data_00003125.png}
    \caption{Energy Oscillation Over Time}
    \label{fig:energy-oscillation-over-time}
\end{figure}
It can be noted that the total energy is not perfectly conserved, though the dissipation due to numerical errors is quite limited with such a small time step. Increasing the time step clearly implies more energy dissipation. Moreover, the version that is run on the GPU device yields results that are consistent with the CPU ones. 

\section{Performance Analysis}
Different performance analyses were performed to assess the scalability of the model. For reference, all tests were conducted on the MPCDF Viper cluster, on the CPU and GPU partitions, respectively. The former is based on the AMD EPYC Genoa 9554 processor, equipped with 128 cores. The latter is based on the MI300A APU, a chip with 24 cores and USM between the CPU and the GPU. Both serial and GPU-accelerated versions were compiled with the \texttt{-O3} optimization option, to ensure consistency of performance comparisons. The time measurement excludes the initialization part and the operation of writing the particle positions and velocities to a file. The former is not of interest, as previously explained, and its execution time is one order of magnitude shorter than the core algorithm, see the table below \ref{tab:ratio_initialization_pullback}. It can be seen that for a sufficiently large number of particle markers, the initialization time corresponds to approximately 6\% of the core algorithm time. The model does not feature MPI parallelization; thus, a single process is used for all simulations. However, the single-core performance of the MI300A is better than that of the former chip, so this should be taken into account when looking at the speedup values. 

\begin{table}[h!] 
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Problem Size} & \textbf{Initialization} & \textbf{Gather-Scatter} \\
\hline
$10^3$ & $8.28\times10^{-4}$ & $3.59\times10^{-3}$ \\
$10^4$ & $3.77\times10^{-3}$ & $4.2\times10^{-2}$ \\
$10^5$ & $3.38\times10^{-2}$ & $5.54\times10^{-1}$ \\
$10^6$ & $3.25\times10^{-1}$ & $5.54$ \\
$10^7$ & $3.22$ & $5.52\times10$ \\
$10^8$ & $3.27\times10$ & $5.51\times10^2$ \\
$10^9$ & $3.20\times10^{2}$ & $5.52\times10^3$ \\
\hline
\end{tabular}
\caption{Configuration of Problem Size, Number of Threads, and Number of Teams}
\label{tab:ratio_initialization_pullback}
\end{table}

\section{Problem Size Scalability}
First of all, a \textbf{problem size scaling analysis} was conducted, which consists of keeping the number of GPU workers fixed, while increasing the problem size, i.e. the particle markers. Specifically, these range from $10^3$ to $10^8$ and increase by one order of magnitude at each step. When it comes to GPU workers, the number of teams is set to 912, whereas the number of threads per team is set to 256. Both values are chosen as the given limit of the MI300A APU architecture. Note that openMP teams are mapped to workgroups, which are analogous to thread blocks on NVIDIA GPUs. Nonetheless, this may vary depending on the compiler implementation of offloading features. In the current case, the maximum number of teams actually corresponds to the number of CUs times the SIMD units per CU, which amounts to $228\times4=912$. The number of threads per team corresponds to the wavefront size multiplied by the number of SIMD units per CU, that is, $64\times4=256$.
Detailed information regarding the architecture and available hardware resources can be found by running the \texttt{rocminfo} command inside a batch script or inside an interactive session. This kind of analysis can be used to assess the efficiency of a fixed GPU configuration for increasing workload size, as well as to simulate the scalability for a given hardware set. 

% TODO: insert the figures and understand why smaller problems can still be solved faster with the max number of teams and threads, while one would expect this to cause too much of an overhead. 
% TODO: could even add some nvidia / rocm profiling to give more insight and details in the kernel execution and data movements
% TODO: remove all the data transfers by leveraging shared memory and check if the performance increases significantly
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{Figures/problem_size_scaling.png}
    \caption{Problem Size Scaling}
    \label{fig:problem-size-scaling}
\end{figure}

Fig. \ref{fig:problem-size-scaling} shows that CPU time grows linearly with respect to the problem size, while the GPU time exhibits a completely different trend. It is clear that for a small problem size, the vast majority is taken by the kernel initialization, regardless of the amount of data to be transferred to the device. Thread creation is expected to be negligible, since GPU threads are created and managed in hardware, unlike CPU threads, which are spawned and scheduled by the OS. This will be assessed in more detail with the strong scalability analysis. 

 \begin{figure}
     \centering
     \includegraphics[width=0.7\linewidth]{Figures/problem_scaling_speedup.png}
     \caption{Problem Size Speedup}
     \label{fig:problem-size-speedup}
 \end{figure}

Fig. \ref{fig:problem-size-speedup} shows the speedup of the GPU kernel with respect to the sequential execution on the CPU. We start obtaining significant speedup when the problem size exceeds one million markers and seems to grow linearly from that size onward. Further simulations should be performed to better assess this, but serial execution takes a significant amount of time. 
TODO: expand the data to at least one billion particle markers, which is an order of magnitude usually used in TRIMEG simulations. This 1D code should exemplify the performance gain that can in principle be obtained with offloading.

\section{Weak Scalability}
Weak scalability consists of keeping the workload per worker constant and progressively increasing both values to evaluate how well an algorithm scales with more computational power. It evaluates how large of a problem can be solved in roughly the same amount of time while increasing the computational resources. The range of problem sizes and the corresponding GPU workers used in the analysis can be found in the table below. Note that the smaller simulations have been run up to 10 times to ensure better consistency of the time measurements. The average execution time as well as the standard deviation are shown in the Fig. \ref{fig:weak-scaling}.
NOTE: the values number of threads per team should be increased up until 1024, while here it stops at 256. Should do the scalability test again with reasonable numbers.

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Problem Size} & \textbf{Num Teams} & \textbf{Num Threads} \\
\hline
$10^3$ & 1 & 1 \\
$10^4$ & 1 & 16 \\
$10^5$ & 1 & 128 \\
$10^6$ & 5 & 256 \\
$10^7$ & 50 & 256 \\
$10^8$ & 500 & 256 \\
\hline
\end{tabular}
\caption{Configuration of Problem Size, Number of Threads, and Number of Teams}
\label{tab:problem_config}
\end{table}

% TODO: insert the figures
Ideally, the line depicting the execution time should be a plateau, which means that there is no additional overhead when adding more work and more computational power to process it, i.e. the workload scales perfectly. Fig. \ref{fig:weak-scaling} does not show the described trend, but this is to be expected since the initialization phase is not accelerated and grows linearly in the number of particle markers. 
TODO: may add another plot that includes only the time spent inside the kernel, that is, for the gather-scatter scheme. This should approximately show the desired trend.

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{Figures/weak_scaling.png}
    \caption{Weak Scaling}
    \label{fig:weak-scaling}
\end{figure}


\section{Strong Scalability}
Strong scalability aims to evaluate how much a task can be accelerated when adding more processing power. Applied to the 1D PIC model, it amounts to fixing the problem size and increase the number of teams and threads per team to see how much of an overhead this implies. The data used for the plots corresponds to fixing the number of particle markers to $10^7$ and doubling the total number of GPU workers for each data point.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/strong_scaling.png}
    \caption{Strong Scaling}
    \label{fig:strong-scaling}
\end{figure}
